Breaking the Bandwidth Barrier: Geometrical Adaptive Entropy Estimation

Estimators of information theoretic measures such as entropy and mutual information are a basic workhorse for many downstream applications in modern data science. State of the art approaches have been either geometric (nearest neighbor (NN) based) or kernel based (with a globally chosen bandwidth). In this paper, we combine both these approaches to design new estimators of entropy and mutual information that outperform state of the art methods. Our estimator uses local bandwidth choices of $k$-NN distances with a finite $k$, independent of the sample size. Such a local and data dependent choice improves performance in practice, but the bandwidth is vanishing at a fast rate, leading to a non-vanishing bias. We show that the asymptotic bias of the proposed estimator is universal; it is independent of the underlying distribution. Hence, it can be pre-computed and subtracted from the estimate. As a byproduct, we obtain a unified way of obtaining both kernel and NN estimators. The corresponding theoretical contribution relating the asymptotic geometry of nearest neighbors to order statistics is of independent mathematical interest.

==> section3_backup_sw.tex <==
We consider {\em  resubstitution} entropy estimators of the form
$\hH(x) = -(1/n)\sum_{i=1}^n \log \hf_n(X_i)$ and  propose to use 
the local likelihood density estimator in \eqref{eq:p2} and
  a  choice of bandwidth that is {\em local} (varying for each point $x$) and {\em adaptive} (based on the data). 
Concretely, we choose, for each sample point $X_i$, the bandwidth $h_{X_i}$ to be the
the distance to its $k$-th nearest neighbor  $\rho_{k,i}$. Precisely,
we propose the following $k$-Local Nearest Neighbor ($k$LNN) entropy estimator of degree-$2$:
\begin{eqnarray}
	\label{eq:resubstitute}
	\hH_{k{\rm LNN}}^{(n)}(X) &=& -\frac{1}{n}\sum_{i=1}^n  \left\{ \log \frac{S_{0,i}}{n(2\pi)^{d/2}\rho_{k,i}^d |\Sigma_i|^{1/2} }
	 - \frac12\frac{1}{S_{0,i}^2}  S_{1,i}^T  \Sigma_i^{-1} S_{1,i} \right\}  - B_{k,d}\;,
\end{eqnarray}
where subtracting $B_{k,d}$ defined in Theorem \ref{thm:unbiased} removes the asymptotic  bias,
and $k\in\Z^+$ is a  hyper parameters determining the bandwidth.
We
only use the $\lceil \log n \rceil$ nearest subset of samples  $\cS_{i}=\{j\in[n]\,:\, j\neq i \text{ and } \|X_i-X_j\|\leq  \rho_{\lceil\log n \rceil,i} \} $  in computing the quantities below:
\begin{eqnarray}
	S_{0,i} \equiv \sum_{j \in \cS_{i,m} } e^{-\frac{\|X_j - X_i\|^2}{2 \rho_{k,i}^2}  } \;, \;\;\;\;
	S_{1,i} \equiv \sum_{j \in \cS_{i,m} } \frac{1}{\rho_{k,i}} (X_j-X_i) e^{-\frac{\|X_j - X_i\|^2}{2 \rho_{k,i}^2}  }\;, \nonumber \\
	S_{2,i} \equiv  \sum_{j \in \cS_{i,m}  } \frac{1}{\rho_{k,i}^2} (X_j-X_i)(X_j-X_i)^T e^{-\frac{\|X_j - X_i\|^2}{2 \rho_{k,i}^2}  }\;,\;\;
	\Sigma_i \equiv \frac{S_{0,i}S_{2,i}- S_{1,i} S_{1,i}^T}{S_{0,i}^2}\;.
	\label{eq:defS}
\end{eqnarray}
The truncation is important in practice
for computational efficiency. % (and also plays a role in the analysis   for  proving Theorem \ref{thm:unbiased}
%and also 
We show in Theorem \ref{thm:unbiased} that the asymptotic bias   is {\em independent} of the underlying distribution and hence can be {\em precomputed} and removed.
% Further, we provide an explicit formula characterizing $B_{k,d}$.
%We provide numerical evaluations in Table \ref{tbl:bias} via sampling and empirically approximating the expectation
%\eqref{eq:defBias}.
\begin{thm}
    \label{thm:unbiased}
    If $k\geq 3$ and $X_1, X_2, \dots, X_n \in \mathbb{R}^d$ are i.i.d.\ samples from
 %   an underlying distribution $P$ with
    a twice continuously differentiable pdf $f(x)$, then
    \begin{eqnarray}
    \lim_{n \to \infty} \E [\hH^{(n)}_{k{\rm LNN}}(X)  ]  &=&  H(X) + B_{k,d} \;,
    \end{eqnarray}
    where $B_{k,d}$ is a  constant that only depends on $k$ and $d$, defined in \eqref{eq:defBias}.
\end{thm}
We relegate the proof to the supplementary material (where for compactness the univariate case is discussed in detail and which can be  generalized to higher dimensions $d$).
Our choice of a local adaptive bandwidth $h_{X_i}=\rho_{k,i}$
is crucial in ensuring that the asymptotic bias $B_{k,d}$
does not  depend on the underlying distribution $f(x)$.
This  relies on a fundamental connection to the theory of asymptotic order statistics made precise in Lemma \ref{lem:order_stat},
which also gives the explicit formula for the bias in \eqref{eq:defBias}.
%This gives the explicit formula for the bias.
%which can be evaluated numerically.
%For multivariate $X$, we conjecture that the asymptotic bias is still independent of $f(x)$, and give a formula for the bias in \eqref{eq:defBias} for general $d$.


The main idea is that the
empirical quantities used in the estimate \eqref{eq:defS}
converge in large $n$ limit to
similar quantities defined over order statistics.
We make this intuition precise in the next section.
We define  order statistics  over
i.i.d.\ standard exponential random variables $E_1,E_2,\ldots,E_m$  and
i.i.d.\ random variables $\xi_1,\xi_2,\ldots,\xi_m$ drawn uniformly (the Haar measure) over the unit sphere in $\reals^d$,
for a variable $m\in\Z^+$. We define for $\alpha\in\{0,1,2\}$,
\begin{eqnarray}
	\tilde{S}^{(m)}_{\alpha}  &\equiv&  \sum_{j=1}^{m} \xi_j^{(\alpha)}\,\frac{ (\sum_{\ell=1}^j E_\ell )^{\alpha}}{(\, \sum_{ \ell=1}^k E_\ell\,)^{\alpha}}
	\exp\left\{- \frac{(\,\sum_{\ell=1}^j E_\ell \,)^{2}}{2(\,\sum_{\ell=1}^k E_\ell\,)^{2}} \right\} \label{eq:S}\;,
\end{eqnarray}
where $\xi_j^{(0)}=1$, $\xi_j^{(1)}=\xi_j\in\reals^d$, and $\xi_j^{(2)}=\xi_j \xi_j^T\in\reals^{d\times d}$, and let
$\tS_\alpha = \lim_{m\to \infty} \tS_\alpha^{(m)}$ and $\tSigma = (1/\tS_0)^2 (\tS_0\tS_2 -\tS_1 \tS_1^T)$.
 We show that the limiting $\tS_\alpha$'s are well-defined (in the proof of Theorem \ref{thm:unbiased}) and are directly related to the bias terms in the resubstitution
 estimator of entropy.  
% When $d=1$, $\xi_j$'s are  Rademacher random variables.

\begin{eqnarray}
	B_{k,d} &=& \E\left[\, \log \left( \sum_{\ell=1}^k E_\ell\right) + \frac{d}{2} \log  2\pi -\log C_d - \log \tS_0 + \frac12 \log  \big|\tSigma \big|  +  \left(\frac{1}{2\tS_0^2} \tS_1^T \tSigma^{-1}\tS_1 \right)  \,\right] \;,
	\label{eq:defBias}
\end{eqnarray}

In practice, we propose using a fixed small $k$ such as five.
For $k\leq3$ the estimator has a very large variance, and
numerical evaluation of the corresponding bias also converges slowly.
For some typical choices of $k$, we provide approximate evaluations below, where
$0.0183(\pm 6)$ indicates empirical mean $0.0183$ with confidence interval   $0.0006$.
In these numerically evaluations, we truncated the summation at $m=50,000$.
Although we prove that $B_{k,d}$ converges in $m$,
in practice, one can choose $m$  based on the number of samples and $B_{k,d}$ can be evaluated for that $m$.


\begin{table}[h]
\begin{center}
  \begin{tabular}{  c c | c | c | c | c | c | c   |}
	\cline{3-8}
    & & \multicolumn{6}{|c|}{$k$} \\ \cline{3-8}
     & &  $4$ & $5$ & $6$ & $7$ & $8$ & $9$ \\ \cline{3-8}   \hline
     \multicolumn{1}{ |c  }{\multirow{2}{*}{$d$} } &
     \multicolumn{1}{ |c|| }{$1$} & -0.0183($\pm$6) & -0.0233($\pm$6) & -0.0220($\pm$4)  & -0.0200($\pm$4) & -0.0181($\pm$4) &  -0.0171($\pm$3)
     % for k=10, -0.0157(3), for k=11, -0.0144(3)
         \\ \cline{2-8}
     \multicolumn{1}{ |c  }{} &
     \multicolumn{1}{ |c|| }{$2$} & -0.1023($\pm$5) & -0.0765($\pm$4) & -0.0628($\pm$4) & -0.0528($\pm$3) & -0.0448($\pm$3)&    -0.0401($\pm$3)  \\ \cline{1-8}
  \end{tabular}
\end{center}
     \caption{Numerically evaluation of $B_{k,d}$, via sampling
       $1,000,000$ instances  for each pair $(k,d)$.}
     \label{tbl:bias}
	\end{table}




 	
%\subsection{}
{\bf Theoretical contribution}: 
Our key technical innovation is
 a fundamental connection
 between nearest neighbor statistics and asymptotic order statistics, stated below as  Lemma \ref{lem:order_stat}: 
we show that the (normalized) distances $\rho_{\ell,i}$'s jointly converge to the standardized uniform  order statistics and
the directions $(X_{j_\ell} -X_i)/\|X_{j_\ell} -X_i\|$'s converge to independent uniform distribution (Haar measure) over the unit sphere.

Conditioned on $X_i=x$,
the proposed estimator uses nearest neighbor statistics on
$Z_{\ell,i} \equiv X_{j_\ell} - x $ where
$X_{j_\ell}$ is the $\ell$-th nearest neighbor from $ x$ such that
$ Z_{\ell,i} = ((X_{j_\ell} -X_i)/\|X_{j_\ell} -X_i\|) \rho_{\ell,i}$.
Naturally, all the  techniques we develop in this paper generalizes to any estimators that depend on
the nearest neighbor statistics $\{Z_{\ell,i}\}_{i,\ell\in[n]}$ -- and the value of such a general result is demonstrated later (in Section~\ref{sec:general}) when we evaluate the bias in similarly inspired entropy estimators \cite{GVG14,GVG15,lombardi2016nonparametric,KL87} from the literature. 

% Consider the joint distribution of $(Z_{1,i},\ldots,Z_{m_n,i})$.
%Fix $X_i = x$. We will show that $\lim_{n \to \infty} \E[H_i | X_i = x] = \log f(x) + C_k$ for some constant $C_k$. Notice that $H_i$ is a function of random variables $ \rho_{k,i}$ and $S_{0,i}, S_{1,i}, S_{2,i}$. Furthermore, $S_{0,i}, S_{1,i}, S_{2,i}$ are functions of $\{\rho_{j,i}\}_{j=1}^{m_n}$. The following lemma gives the distribution of $\{\rho_{j,i}\}_{j=1}^{m_n}$ as $n$ goes to infinity.
\begin{lemma}
    \label{lem:order_stat}
    Let $E_1, E_2, \dots, E_{m_n}$ be i.i.d.\ standard exponential random variables and
    $\xi_1 , \xi_2, \dots, \xi_{m_n}$ be i.i.d.\ random variables  drawn uniformly over the unit $(d-1)$-dimensional sphere
    in $d$ dimensions,
    independent of the $E_i$'s.
    Suppose we have a uniform bound over all $x\in\reals$ on $f''(x)/(f(x))^3 =O(1)$ and $f'(x)/f(x) = O(1)$, then for
    any $m_n = O( \log n)$,
    we have the following convergence  conditioned on  $X_i = x$:
    \begin{eqnarray}
    \lim_{n \to \infty} d_{\rm TV} \left( 2nf(x)\Big(\, Z_{1,i}, Z_{2,i}, \dots, Z_{m_n,i} \,\Big) \;,\;
    \left(\, \xi_1 E_1, \xi_2(E_1 + E_2), \dots , \xi_{m_n}\sum_{\ell=1}^{m_n} E_\ell \,\right) \right) = 0 \;.
    \end{eqnarray}
    where $d_{\rm TV}(\cdot,\cdot)$ is the total variation between two random variables.%$\|X - Y\|_{TV} = \sup_B |\,\Pr\{X \in B\} - \Pr\{Y \in B\}\,|$ is the total variation distance of two random variables $X$ and $Y$.
\end{lemma}

%Given this, ...

{\bf Empirical contribution}:  
 Numerical experiments suggests that the proposed estimator
outperforms 
state-of-the-art entropy estimators, 
and the gap increases with correlation.  
The idea of using $k$NN distance as bandwidth 
for entropy estimation was originally proposed 
by Kozachenko and Leonenko in  \cite{KL87}. 
This estimator, which we dub KL estimator, 
resubstitutes \eqref{eq:knn} to estimate entropy, 
and is a special case of the $k$LNN method we propose with degree $0$ and a step kernel. 
We refer to Section \ref{sec:general} for a formal comparison.
One of the most popular estimator is 
using KDE in \eqref{eq:p0} and resubstituting it to estimate entropy \cite{Joe89}. 
This is a special case of the  $k$LNN method with degree $0$, and 
the Gaussian kernel is used in simulations. 
Recently, a new estimator based on von Mises expansion 
was introduced in \cite{KKPW15}, which achieves improved convergence rate in the large sample regime. 
In Figure \ref{fig:entropy} (left), we draw $100$ samples i.i.d. from two standard Gaussian random variables with correlation $r$, and plot resulting  mean squared error averaged over $100$ instances.  
The ground truth, in this case is  $H(X) = \log(2 \pi e) + 0.5 \log(1-R^2)$.
% N = 500, truncation = 80
On the right, we repeat the same simulation for fixed $r=0.99999$ and varying number of samples. 
 
\begin{figure}[h]
	\begin{center}
	\includegraphics[width=.45\textwidth]{entropy}
	\put(-220,70){$ E[(\hH-H)^2] $}
	\put(-140,-10){ $(1-r)$ where $r$ is correlation}
	\includegraphics[width=.45\textwidth]{entropy_fixed_r}
	\put(-120,-10){number of samples $n$}
	\end{center}
	\caption{Degree-2 $k$LNN  outperforms other state-of-the-art estimators for entropy estimation. }
	\label{fig:entropy}
\end{figure}


==> supplementary_backup.tex <==
\subsection{Proof of proposition \ref{pro:closedform} }
\label{proof:prop}
We first prove the  derivation of the LLDE with degree $p=2$ in Equation \eqref{eq:p2}.
The gradient of the local likelihood evaluated at the  maximizer is zero \cite{Loa96}, which gives a computational tool for finding the maximizer:
\begin{align}
& \frac{1}{n} \sum_{j=1}^{n} K(\frac{X_j - x}{h}) = \int K(\frac{u-x}{h}) e^{a_0 + a_1^T (u-x) + (u-x)^T a_2 (u-x)} du \;,\label{eq:ll_0}\\
& \frac{1}{n} \sum_{j=1}^{n} \frac{X_j - x}{h} K(\frac{X_j - x}{h}) = \int \frac{u-x}{h} K(\frac{u-x}{h}) e^{a_0 + a_1^T (u-x) + (u-x)^T a_2 (u-x)} du \;,\label{eq:ll_1}\\
& \frac{1}{n} \sum_{j=1}^{n} \frac{(X_j - x)(X_j - x)^T}{h^2} K(\frac{X_j - x}{h}) \nonumber \\
&\;\;\;\; = \int \frac{(u-x)(u-x)^T}{h^2} K(\frac{u-x}{h}) e^{a_0 + a_1^T (u-x) + (u-x)^T a_2 (u-x)} du \;,\label{eq:ll_2}
\end{align}
where $K(x) = \exp\{-\|x\|^2/2\}$ is the Gaussian kernel.
Notice that the left-hand side of the equations are $S_0/n$, $S_1/n$ and $S_2/n$, respectively.
The RHS can be written in closed forms as:
\begin{eqnarray}
\frac{1}{n}S_0 &=& (2\pi)^{d/2} |{M}|^{-1/2} e^{a_0+\frac{1}{2}a_1^TM^{-1}a_1 } \;,\label{eq:ll'_0}\\
\frac{1}{n}S_1 &=& \frac{1}{nh} S_0  M^{-1} a_1\;,\label{eq:ll'_1}\\
\frac{1}{n}S_2 &=& \frac{1}{nh^2} S_0  (M^{-1} +  M^{-1}a_1a_1^TM^{-1})\;,\label{eq:ll'_2}
\end{eqnarray}
where $M = h^{-2} I_{d \times d} - 2a_2$ assuming $h$ sufficiently small such that $M$ is positive definite.
We want to derive $\hat{f}(x) = \exp\{a_0\}$ from the equations.
From \eqref{eq:ll'_1}  we get $M^{-1}a_1 = S_1(h/S_0)$.
Together with \eqref{eq:ll'_2},
we get $M^{-1} + M^{-1}a_1a_1^TM^{-1} = S_2(h^2/S_0)$.
Hence, $M^{-1} = (S_2/S_0 - (S_1/S_0) (S_1/S_0)^T) h^2 =  h^2 \Sigma $.
Plug them in~\eqref{eq:ll'_0}, we obtain the desired expression.
%\begin{eqnarray}
%\hat{f}(x) %&=& \exp\{a_0\} = \frac{S_0}{n (2\pi)^{d/2} (\det{M})^{-1/2}} \exp\{-\frac{1}{2} a_1^T M^{-1} a_1\} \,\notag\\
%&=&  \frac{S_0}{n (2\pi)^{d/2} (\det{M})^{-1/2}} \exp\{-\frac{1}{2} (M^{-1}a_1)^T M (M^{-1}a_1)\} \,\notag\\
%&=& \frac{S_0}{n (2\pi)^{d/2} |\Sigma|^{1/2} h^d} \exp\Big\{-\frac{1}{2S_0^2} (S_1^T \Sigma^{-1} S_1) \Big\} \;.
%\end{eqnarray}

% ---------------------------------------------------------------------------------------------------------------------------------
Analogously, for the derivation of the LLDE with degree $p=1$ in Equation \eqref{eq:p1}, we get
\begin{eqnarray}
\frac{1}{n}S_0 &=& (2\pi)^{d/2} h^{d} e^{a_0+\frac{h^2}{2}a_1^Ta_1 } \;,\label{eq:ll'_10}\\
\frac{1}{n}S_1 &=& \frac{h}{n} S_0   a_1\label{eq:ll'_11}\;.
\end{eqnarray}
This gives $a_1=(1/(hS_0))S_1$, and
$e^{a_0} = (S_0/(n(2\pi)^{d/2} h^{d}))\,\exp\{-0.5\|S_1\|^2/S_0^2\}$.

% -------------------------------------------------------------------------------------------------------------------------------------
\section{Proof of Lemma~\ref{lem:order_stat}}
\label{sec:order_stat}

Let us introduce some notations first.
Define $S^{d-1} \equiv \{x \in \mathbb{R}^d: \|x\| = 1\}$ as the unit $(d-1)$-dimensional sphere and $\sigma^{d-1}$ as a normalized spherical measure on $S^{d-1}$.
For any $\theta = (\theta_1, \dots, \theta_m) \in (S^{d-1})^m$ and $x = (x_1, \dots, x_m) \in \mathbb{R}_+^m$, define $\theta x \equiv (\theta_1 x_1, \dots, \theta_m x_m) \in \mathbb{R}^{d \times m}$.
For any set $B \in \mathbb{R}^{d \times m}$ and $\theta \in (S^{d-1})^m$, define $B_{\theta} = \{x \in \mathbb{R}_+^m: \theta x \in B\}$.
Let $\{\xi_i\}_{i=1}^m$ be i.i.d. random variables uniformly over $S^{d-1}$. Then for any joint random variables $(W_1, \dots, W_m) \in \mathbb{R}_+^m$ which are independent with $\{\xi_i\}_{i=1}^m$, we have
\begin{eqnarray}
\Pr\{ (\xi_1 W_1, \dots, \xi_m W_m) \in B\} &=& \int_{\theta \in (S^{d-1})^m } \Pr\{ (W_1, \dots, W_m) \in B_{\theta} \,|\, \theta\} \, d(\sigma^{d-1})^m(\theta) \;.
\end{eqnarray}

Let $Z=(Z_{1,i},\ldots,Z_{m,i})$, $\|Z\|=( \|Z_{1,i}\| ,\ldots, \|Z_{m,i}\|)$ and let $E=( E_1^{1/d} ,\ldots, (\sum_{\ell=1}^m E_\ell)^{1/d})$, then
\begin{eqnarray}
&&\left|\, \Pr\left\{\, (c_d nf(x))^{1/d} Z \in B \,\right\} - \Pr\left\{\,\left(\, \xi_1 E_1^{1/d}, \dots, \xi_m (\sum_{\ell=1}^m E_\ell)^{1/d} \,\right) \in B \,\right\} \,\right| \,\notag\\
&\leq&  \left|\, \Pr\left\{\, (c_d nf(x))^{1/d} Z \in B \,\right\} - \int_{\theta \in (S^{d-1})^m } \Pr\{ (E_1^{1/d}, \dots, (\sum_{\ell=1}^m E_\ell)^{1/d}) \in B_{\theta} \,|\, \theta\} \, d(\sigma^{d-1})^m(\theta) \,\right| \,\notag\\
&\leq& \left|\, \Pr\left\{\, (c_d nf(x))^{1/d} Z \in B \,\right\} - \int_{\theta \in (S^{d-1})^m } \Pr\{ (c_d nf(x))^{1/d} \|Z\| \in B_{\theta} \,|\, \theta\} \, d(\sigma^{d-1})^m(\theta) \,\right| \,\notag\\
&+& \int_{\theta \in (S^{d-1})^m} \left|\, \Pr\{ (c_d nf(x))^{1/d} \|Z\| \in B_{\theta} \,|\, \theta\} - \Pr\{ E \in B_{\theta} \,|\, \theta \} \,\right| d(\sigma^{d-1})^m(\theta) \;.\label{eq:tv}
\end{eqnarray}

Now consider the first term in~\eqref{eq:tv}. %To simplify the notations, let $\mathcal{E}_{\lambda}$ be the event of $\left(\, 2nf(x)Z_{1,i}, \dots, 2nf(x)Z_{m,i} \,\right) \in B_{\lambda}$ and $\mathcal{E}'_{\lambda}$ be the event of $\left(\, 2nf(x)|Z_{1,i}|, \dots, 2nf(x)|Z_{m,i}| \,\right) \in |B_{\lambda}|$.
We consider two cases separately.

{\bf Case 1.} If $\|Z_{m,i}\| \geq (\sqrt{n} c_d f(x))^{-1/d}$, we show that the tail events happen with a low probability. Denote $B(x,r) = \{z: \|z-x\| \leq r\}$ and let $p = \Pr\{t \in B(x, \|Z_{m,i}\|)\} = \int_{B(x,\|Z_{m,i}\|)} f(t) dt$. Since $f$ is twice continuously differentiable, we can see that $p \geq 0.5 c_d \|Z_{m,i}\|^d f(x) \geq 0.5/\sqrt{n}$ for sufficiently large $n$. Therefore,
\begin{eqnarray}
\Pr\{\|Z_{m,i}\| \geq (\sqrt{n} c_d f(x))^{-1/d}\} &=& \sum_{\ell=0}^{m-1} {n \choose \ell} p^{\ell} (1-p)^{n-\ell} \leq \sum_{\ell=0}^{m-1} n^{\ell} \Big(1-\frac{1}{2\sqrt{n}}\Big)^{(n-\ell)} \,\notag\\
&\leq& \sum_{\ell=0}^{m-1} n^l e^{-(\sqrt{n} - \ell\sqrt{n})/2} \leq m n^m e^{-(\sqrt{n} - m/\sqrt{n})/2} \;.
\end{eqnarray}

{\bf Case 2.} If $\|Z_{m,i}\| < (\sqrt{n} c_d f(x))^{-1/d}$, let $\overline{B} = \{t: (c_d n f(x))^{1/d} t \in B \textrm{ and } \|t_m\| < (\sqrt{n} c_d f(x))^{-1/d} \}$ and $\overline{B_{\theta}} = \{t: (c_d n f(x))^{1/d} t \in B_{\theta} \textrm{ and } t_m < (\sqrt{n} c_d f(x))^{-1/d} \}$.
Note that 
\begin{eqnarray}
\Pr (Z \in \tA) = (n!/(n-k)!)\int_{t\in\tA} \prod_{j=1}^m f(x+t_j) \Pr_X(|X-x|>|t_m|)^{n-m} dt \;,
\end{eqnarray}
which gives
\begin{eqnarray}
&& \frac{\int_{\theta \in (S^{d-1})^m} \Pr\{(c_d n f(x))^{1/d}\|Z\| \in B_{\theta}, \|Z_{m,i}\| < (\sqrt{n} c_d f(x))^{-1/d} \,|\,\theta\} \, d(\sigma^{d-1})^m(\theta)}{\Pr\{(c_d n f(x))^{1/d} Z \in B, \|Z_{m,i}\| < (\sqrt{n} c_d f(x))^{-1/d}\}} \,\notag\\
&=& \frac{\int_{\theta \in (S^{d-1})^m} \Pr\{\|Z\| \in \overline{B_{\theta}} \,|\,\theta\} \, d(\sigma^{d-1})^m(\theta)}{\Pr\{ Z \in \overline{B}\}} \,\notag\\
&=& \frac{\int_{\theta \in (S^{d-1})^m} \frac{n!}{(n-k)!} \left(\, \int_{t \in \overline{B_{\theta}}} \left(\, \prod_{j=1}^m f(x + \theta_j t_j) \,\right)\, \left(\, \Pr\{\|X-x\| > \|t_m\|\} \,\right)^{n-m} dt \,\right)\, d(\sigma^{d-1})^m(\theta) }{ \frac{n!}{(n-k)!} \int_{t \in \overline{B}} \left(\, \prod_{j=1}^m f(x + t_j) \,\right)\, \left(\, \Pr\{\|X-x\| > \|t_m\|\} \,\right)^{n-m} dt} \,\notag\\
&\leq& \frac{\sup_{\theta \in (S^{d-1})^m} \sup_{t \in \overline{B_{\theta}}} \prod_{j=1}^m f(x+ \theta_j t_j)}{\inf_{t \in \overline{B}} \prod_{j=1}^m f(x+t_j)} \, \notag\\
&\leq& \left(\, \frac{\sup_{\|t\| \leq (\sqrt{n} c_d f(x))^{-1/d}} f(x+t)}{\inf_{\|t\| \leq (\sqrt{n} c_d f(x))^{-1/d}} f(x+t )}\,\right)^m \;,\label{eq:ratio}
\end{eqnarray}

where the first inequality follows from the fact that
$\int_{\theta \in (S^{d-1})^m} ( \int_{\overline{B_\theta}} g(t_m)dt ) d (\sigma^{d-1})^m (\theta) = \int_{\overline{B}} g(\|t_m\|)dt$.
Since $f$ is continuously differentiable, by mean value theorem, there exists $a, b \in B(x, (\sqrt{n} c_d f(x))^{-1/d})$ such that
\begin{eqnarray}
\frac{\sup_{\|t\| \leq (\sqrt{n} c_d f(x))^{-1/d}} f(x+t)}{\inf_{\|t\| \leq (\sqrt{n} c_d f(x))^{-1/d}} f(x+t )} &=& \frac{f(b) + (a-b)^T \nabla f(a) }{f(b)} \leq 1 + \frac{2 (\sqrt{n} c_d f(x))^{-1/d} \|\nabla f(a)\|}{f(b)} \;,
\end{eqnarray}
By the assumption, there exists a ball $B(x,\varepsilon)$ such that $\|\nabla f(a)\| = O(1)$ and $f(a) > 0$ for all $a \in B(x, \varepsilon)$, so for sufficiently large $n$ such that $(\sqrt{n} c_d f(x))^{-1/d} < \varepsilon$, there exists some constant $C$ such that $\sup_{\|t\| \leq (\sqrt{n} c_d f(x))^{-1/d}} f(x+t) \leq (1 + C n^{-1/(2d)}) \inf_{\|t\| \leq (\sqrt{n} c_d f(x))^{-1/d}} f(x+t )$. Therefore,~\eqref{eq:ratio} is upper bounded by $(1 + C n^{-1/(2d)})^m$. Similarly,~\eqref{eq:ratio} is lower bounded by $(1 - C n^{-1/(2d)})^m$.

For simplicity, let $\mathcal{E} = \{\|Z_{m,i}\| < (\sqrt{n} c_d f(x))^{-1/d}\}$. Then combining the two cases, the first term in~\eqref{eq:tv} is bounded by:
\begin{eqnarray}
&& \left|\, \Pr\left\{\, (c_d nf(x))^{1/d} Z \in B \,\right\} - \int_{\theta \in (S^{d-1})^m } \Pr\{ (c_d nf(x))^{1/d} \|Z\| \in B_{\theta} \,|\, \theta\} \, d(\sigma^{d-1})^m(\theta) \,\right| \,\notag\\
&\leq& \Pr\left\{\, (c_d nf(x))^{1/d} Z \in B, \mathcal{E}^C \,\right\} + \int_{\theta \in (S^{d-1})^m } \Pr\{ (c_d nf(x))^{1/d} \|Z\| \in B_{\theta}, \mathcal{E}^C \,|\, \theta\} \, d(\sigma^{d-1})^m(\theta) \,\notag\\
&+& \left|\, \Pr\left\{\, (c_d nf(x))^{1/d} Z \in B, \mathcal{E}\,\right\} - \int_{\theta \in (S^{d-1})^m } \Pr\{ (c_d nf(x))^{1/d} \|Z\| \in B_{\theta}, \mathcal{E} \,|\, \theta\} \, d(\sigma^{d-1})^m(\theta) \,\right| \,\notag\\
&\leq& \Pr\{\mathcal{E}^C\} + \int_{\theta \in (S^{d-1})^m } \Pr\{ \mathcal{E}^C \} \, d(\sigma^{d-1})^m(\theta) \,\notag\\
&+& \Pr\left\{\, (c_d nf(x))^{1/d} Z \in B, \mathcal{E}\,\right\} \, \left|\, 1 -  \frac{\int_{\theta \in (S^{d-1})^m } \Pr\{ (c_d nf(x))^{1/d} \|Z\| \in B_{\theta}, \mathcal{E} \,|\, \theta\} \, d(\sigma^{d-1})^m(\theta)}{\Pr\left\{\, (c_d nf(x))^{1/d} Z \in B, \mathcal{E}\,\right\}}\,\right| \,\notag\\
&\leq& 2 \Pr\{\mathcal{E}^C\} + \Pr\left\{\, (c_d nf(x))^{1/d} Z \in B, \mathcal{E}\,\right\} \max\{(1+Cn^{-1/(2d)})^m - 1, 1 - (1-Cn^{-1/(2d)})^m\} \,\notag\\
&\leq& 2 m n^m e^{-(\sqrt{n} - m/\sqrt{n})/2} + \max\{(1+Cn^{-1/(2d)})^m - 1, 1 - (1-Cn^{-1/(2d)})^m\} \;.\label{eq:ub100}
\end{eqnarray}


Now consider the second term of~\eqref{eq:tv}. We will use Corollary 5.5.5 of ~\cite{Rei12} to show that
this term vanishes for $m=O(\log n)$ and as $n$ grows.

\begin{lemma}[Corollary 5.5.5, ~\cite{Rei12}]
    \label{lem:reiss}
    Let $Y_1, Y_2, \dots, Y_n$ be i.i.d. samples from unknown distribution with pdf $f$. Let $Y_{1:n} \leq Y_{2:n} \leq \dots \leq Y_{n:n}$ be the order statistics. Assume the density $f$ satisfies $|\log f(y)| \leq L y^{\delta}$ for $0 < y < y_0$ and $f(y) = 0$ for $y < 0$, where $L$ and $\delta$ are constants. Then
    \begin{eqnarray}
        d_{\rm TV}\Big(\, n\,\left(\,Y_{1:n}, Y_{2:n}, \dots, Y_{m:n}\right) , \big(\,E_1, E_1+E_2, \dots, \sum_{j=1}^m E_j\big) \,\Big)  \leq C_0 \left(\, (m/n)^{\delta} m^{1/2} + m/n \,\right) \;,
    \end{eqnarray}
    where $C_0 > 0$ is a constant. $E_1, \dots, E_m$ are i.i.d standard exponential random variables.
\end{lemma}

Now for fixed $x$, consider the distribution of $c_d f(x)\|X - x\|^d$ denoted by $\tilde{P}$. Define $Y_1, Y_2, \dots, Y_n$ drawn i.i.d. from $\tilde{P}$. We can see that $c_d f(x) \|Z\|^d \stackrel{\mathcal{L}}{=} (Y_{1:n}, \dots, Y_{m:n})$, where $\stackrel{\mathcal{L}}{=}$ denotes equivalence in distribution. The pdf $\tilde{f}$ of $\tilde{P}$ is given by:
\begin{eqnarray}
\tilde{f}(t) = \frac{d}{dt} \Pr\{c_d f(x)\|X - x\|^d \leq t\} = \frac{d}{dt} \int_{y \in B(x, r_t)} f(y) dy  \;.
\end{eqnarray}
where $r_t = (t/(c_d f(x)))^{1/d}$. Here we have:
\begin{eqnarray}
\frac{dr_t}{dt} = \frac{t^{1/d-1} (c_d f(x))^{-1/d}}{d} = \frac{1}{f(x) d c_d r_t^{d-1}} \;.
 \end{eqnarray}
 If $f$ is twice continuously differentiable, we have:
\begin{eqnarray}
\left|\, \tilde{f}(t) - 1 \,\right| &=& \left|\, \frac{d}{dt} \int_{y \in B(x, r_t)} f(y) dy - 1 \,\right| = \left|\, \frac{dr_t}{dt} (\frac{d}{dr_t} \int_{y \in B(x, r_t)} f(y) dy) - 1 \,\right| \,\notag\\
&=& \frac{1}{f(x) d c_d r_t^{d-1}} \left|\, \frac{d}{dr_t} \left(\, \int_{y \in B(x,r_t)} f(y) dy \,\right)- f(x) d c_d r_t^{d-1} \,\right| \,\notag\\
&=& \frac{1}{f(x) d c_d r_t^{d-1}} \left|\, \int_{y \in S^{d-1}(x,r_t)} (f(y) - f(x)) d\sigma^{d-1}(y) \,\right| \;,
\end{eqnarray}
where $S^{d-1}$ is the $(d-1)$-sphere centered at $x$ with radius $r_t$ and $\sigma^{d-1}$ is the spherical measure. By mean value theorem, there exists $a(y) \in B(x,r_t)$ such that $f(y) - f(x) = (y-x)^T \nabla f(x) + (a(y)-x)^T H_f(a(y)) (a(y)-x)$, where $a(y)$ depends on $y$. Therefore,
\begin{eqnarray}
&& \left|\, \int_{y \in S^{d-1}(x,r_t)} (f(y) - f(x)) d\sigma^{d-1}(y) \,\right| \,\notag\\
&=& \left|\, \underbrace{\int_{y \in S^{d-1}(x,r_t)} (y-x)^T \nabla f(x)  d\sigma^{d-1}(y)}_{=0} + \int_{y \in S^{d-1}(x,r_t)} (a(y)-x)^T H_f(a(y)) (a(y)-x)  d\sigma^{d-1}(y)\,\right| \,\notag\\
&\leq& \left(\, \sup_{a \in B(x,r_t)} \|H_f(a)\| \, \|a-x\|^2 \,\right) \sigma^{d-1}(S^{d-1}(x,r_t)) \,\notag\\
&\leq& d c_d r_t^{d+1} \left(\, \sup_{a \in B(x,r_t)} \|H_f(a)\| \,\right)
\end{eqnarray}
Since there exists a ball $B(x,\varepsilon)$ such that $\|H_f(a)\| = O(1)$ for all $a \in B(x, \varepsilon)$. Therefore, for sufficiently small $t$ such that $r_t < \varepsilon$, we have:
\begin{eqnarray}
\left|\, \tilde{f}(t) - 1 \,\right| \leq \frac{d c_d r_t^{d+1} \left(\, \sup_{a \in B(x,r_t)} \|H_f(a)\| \,\right)}{f(x) d c_d r_t^{d-1}} = \frac{r_t^2 \left(\, \sup_{a \in B(x,r_t)} \|H_f(a)\| \,\right)}{f(x)} \;.
\end{eqnarray}
Recall that $r_t = (t/(c_df(x)))^{1/d}$, so there exists $L > 0$ such that $|\tilde{f}(t) - 1| \leq L t^{2/d}$ for sufficiently small $t$. Hence, $|\log \tilde{f}(t)| \leq L' t^{2/d}$ for some $L'>0$ and sufficiently small $t$.
 So $\tilde{f}$ satisfies the condition in Lemma.~\ref{lem:reiss} with $\delta = 2/d$. Therefore, for any $B_{\theta} \subseteq \mathbb{R}_+^m$, we have:
\begin{eqnarray}
&&\left|\, \Pr\{ (c_d nf(x))^{1/d} \|Z\| \in B_{\theta} \} - \Pr\{ E \in B_{\theta}\} \,\right| \,\notag\\
&\leq& d_{\rm TV} \left(\, c_d n f(x) \|Z\|^d, \big(\,E_1, E_1+E_2, \dots, \sum_{j=1}^m E_j\big) \,\right) \,\notag\\
&\leq& C_0\left(\, (\frac{m}{n})^{2/d} m^{1/2} + \frac{m}{n} \,\right) \;.\label{eq:ub200}
\end{eqnarray}
Therefore, by combing~\eqref{eq:ub100} and~\eqref{eq:ub200}, we have:
\begin{eqnarray}
&&\left|\, \Pr\left\{\, (c_d nf(x))^{1/d} Z \in B \,\right\} - \Pr\left\{\,\left(\, \xi_1 E_1^{1/d}, \dots, \xi_m (\sum_{l=1}^m E_{\ell})^{1/d} \,\right) \in B \,\right\} \,\right| \,\notag\\
&\leq& 2 m n^m e^{-\frac{\sqrt{n} - m/\sqrt{n}}{2}} + \max\{(1+Cn^{\frac{-1}{2d}})^m - 1, 1 - (1-Cn^{\frac{-1}{2d}})^m\} + C_0\left(\, (\frac{m}{n})^{\frac{2}{d}} m^{\frac{1}{2}} + \frac{m}{n} \,\right)\;,
\end{eqnarray}
for any set $B \in \mathbb{R}^{d \times m}$. Therefore, the total variation distance $d_{\rm TV} ( (c_d nf(x))^{1/d} (\, Z_{1,i}, Z_{2,i}, \dots, Z_{m,i} ) ,( \xi_1 E_1^{1/d}, \xi_2(E_1 + E_2)^{1/d}, \dots , \xi_{m}(\sum_{\ell=1}^{m} E_\ell)^{1/d} \,) )$ is bounded by the RHS quantity. By taking $m = O(\log n)$, the RHS converges to 0 as $n$ goes to infinity. Therefore, we have the desired statement.





% ---------------------------------------------------------------------------------------------------------------------------------
\section{Proof of Theorem \ref{thm:unbiased}}
\label{sec:proofmaintheorem}
We first compute the asymptotic bias.
We define new notations to represent the estimate as
\begin{eqnarray*}
	\hH^{(n)}_k=\frac1n \sum_{i=1}^n \Big\{ \underbrace{\bh\big(\,(c_d nf(X_i))^{1/d} Z_{k,i}, S_{0,i}, S_{1,i}, S_{2,i})\,\big) - \log f(X_i)}_{\equiv H_i}  \Big\} \;,
\end{eqnarray*}
where  $\bar{h} : \mathbb{R}^d \times \mathbb{R} \times \mathbb{R}^d \times \mathbb{R}^{d \times d} \to [-10^{10}, 10^{10}]$ is defined from
\begin{align}
&h(t_1, t_2, t_3, t_4) = \nonumber\\
&\;\;d \log \|t_1\| + d \log (2 \pi) - \log c_d - \log t_2  + \frac{1}{2} \log \left(\, \det\left(\, \frac{t_4}{t_2} - \frac{t_3 t_3^T}{t^2_2}\,\right) \,\right)+ \frac{1}{2} t_3^T (t_4 - t_3 t_3^T)^{-1} t_3 \;,
\end{align}
and $\bar{h} = h$ if $|h| < 10^{10}$, $\bar{h} = 10^{10}$ if $h > 10^{10}$ and $\bar{h} = -10^{10}$ if $h < -10^{10}$. Such a truncation is necessary for exchanging the limit.
%Therefore,  $\bar{h}( 2nf(x)\rho_{k,i}, S_{0,i}, S_{1,i}, S_{2,i}) = H_i + \log f(x)$.
Let $H_i \equiv \bh((c_dnf(X_i))^{1/d}Z_{k,i}, S_{0,i}, S_{1,i}, S_{2,i}))  - \log f(X_i)$.
 Since the terms $H_1, H_2, \dots, H_n$ are identically distributed, the expected value of $\hH_k^{(n)}$ converges to
\begin{eqnarray}
	 \label{eq:entropy1}
    \lim_{n \to \infty} \E[\hH_k^{(n)}] &=& \lim_{n \to \infty} \E[H_1] \,  \;\;=\;\;
    \E_{X_1} \left[\, \lim_{n \to \infty} \E[H_1|X_1] \,\right] \,,
%    &=& \E_{X_1} [-\log f(X_1) + C_{k,m}] \,\notag\\
 %   &=& H(P) + C_k \;.
\end{eqnarray}
where we apply the dominated convergence theorem to exchange the limit and expectation over $X_1$, since  $|H_1| < 10^{10}$.
Perhaps surprisingly, we will show that the expectation inside converges to $-\log f(X_1)$ plus some bias that is independent of the underlying distribution. Precisely, for almost every $x$ and given $X_1 = x$,
\begin{eqnarray}
\E[H_1 | X_1 = x] + \log f(x) &=& \E \left[\, \bar{h}( (c_d nf(x))^{1/d} Z_{k,i}, S_{0,1}, S_{1,i}, S_{2,i}) \,\right] \,\notag\\
& \longrightarrow & B_{k,d}\;,
\label{eq:entropy2}
%\E\left[\, \bar{h} \left(\,\xi_k \sum_{l=1}^k E_\ell, \tilde{S}^{(\infty)}_{0,i}, \tilde{S}^{(\infty)}_{1,i}, \tilde{S}^{(\infty)}_{2,i} \,\right) \,\right] \;,
\end{eqnarray}
as $n\to \infty$ where $B_{k,d}$  is a constant  that only depends on $k$ and $d$, defined in \eqref{eq:defB}. This implies that
\begin{eqnarray}
    \E_{X_1} \left[\, \lim_{n \to \infty} \E[H_1|X_1]\right] & =&     \E_{X_1} [-\log f(X_1) + B_{k,d}] \,\notag\\
    &=& H(X) + B_{k,d} \;.\label{eq:entropy4}
\end{eqnarray}
Together with \eqref{eq:entropy1}, this finishes the proof of the desired claim.

We are now left to prove the convergence of  \eqref{eq:entropy2}. We first give a formal definition of
the bias $B_{k,d}$ by replacing the sample defined quantities by a similar quantities defined from order-statistics,
and use Lemma \ref{lem:order_stat} to prove the convergence.
Recall that our order-statistics is defined by two sequences of $m$ i.i.d. random variables:
i.i.d. standard exponential random variables $E_1, \dots, E_m$ and
i.i.d. random variables  $\xi_1, \dots, \xi_m$ uniformly distributed over $S^{d-1}$.
We define
\begin{eqnarray}
	\label{eq:defB}
	B_{k,d} &\equiv &
	\E\left[\, \bar{h} \left(\,\xi_k \left(\, \sum_{\ell=1}^k E_\ell \,\right)^{1/d}, \tilde{S}^{(\infty)}_{0}, \tilde{S}^{(\infty)}_{1}, \tilde{S}^{(\infty)}_{2} \,\right) \,\right] \;,
\end{eqnarray}
where, as we will show,
$\tS_\alpha^{(\infty)}$ is the limit of empirical quantity $S_{\alpha,i}$ defined from samples for each $\alpha\in\{0,1,2\}$,
and we know that $(c_d nf(x))^{1/d} Z_{k,i}$ converges to $\xi_k (\sum_{\ell=1}^k E_\ell)^{1/d}$ for almost every $x$ from Lemma \ref{lem:order_stat}.
$S^{(\infty)}$ is defined by a convergent random sequence
\begin{eqnarray}
\tilde{S}^{(m)}_{\alpha}  &\equiv&  \sum_{j=1}^{m} \frac{\xi_j^{(\alpha)} (\sum_{\ell=1}^j E_\ell)^{\alpha/d} }{(\sum_{\ell=1}^k E_\ell)^{\alpha/d} } \exp\Big\{- \frac{(\,\sum_{\ell=1}^j E_\ell\,)^{2/d}}{2(\,\sum_{\ell=1}^k E_\ell \,)^{2/d}} \Big\} \;,
\end{eqnarray}
where $\xi_j^{(0)} = 1$, $\xi_j^{(1)} = \xi_j$, $\xi_j^{(2)} = \xi_j \xi_j^T$ and $\tS^{(\infty)}_\alpha = \lim_{m\to \infty} \tS^{(m)}_\alpha$.
This limit exists, since $\tS_0^{(m)}$ is non-decreasing in $m$,
and the convergence of $\tS_1^{(m)}$  and $\tS_2^{(m)}$ follows from Lemma  \ref{lem:tail}.
We introduce simpler notations for the joint random variables:
$\tS^{(m)}=(\xi_k (\sum_{\ell=1}^k E_{\ell})^{1/d}, \tilde{S}^{(m)}_{0},\tilde{S}^{(m)}_{1},\tilde{S}^{(m)}_{2})$ and
 $\tS^{(\infty)}=(\xi_k (\sum_{\ell=1}^k E_{\ell})^{1/d}, \tilde{S}^{(\infty)}_{0}, \tilde{S}^{(\infty)}_{1}, \tilde{S}^{(\infty)}_{2})$.
Considering the quantities  $S^{(n)} = ((c_d nf(x))^{1/d} Z_{k,i}, S_{0,i}, S_{1,i}, S_{2,i})$
defined from samples, we show that this converges
to $\tS^{(\infty)}$.
Precisely, applying  triangular inequality,
\begin{eqnarray}
	d_{\rm TV} (S^{(n)},\tS^{(\infty)}) &\leq&
	d_{\rm TV} (S^{(n)},\tS^{(m)}) + d_{\rm TV} (\tS^{(m)},\tS^{(\infty)}) \;, \label{eq:entropy3}
%	&=&d_{\rm TV} (S^{(n)},\tS^{(m)})  + d_{\rm TV}((\tS_0^{(m)},\tS_1^{(m)},\tS_2^{(m)}),(\tS_0^{(\infty)},\tS_1^{(\infty)},\tS_2^{(\infty)})) \nonumber\;.,
\end{eqnarray}
%&& \Big\| (2nf(x) \rho_{k,i}, S_{0,i}, S_{1,i}, S_{2,i}) - (\xi_k \sum_{l=1}^k E_\ell, \tilde{S}^{(\infty)}_{0,i}, \tilde{S}^{(\infty)}_{1,i}, \tilde{S}^{(\infty)}_{2,i})\Big\|_{TV} \,\notag\\
%&\leq& \Big\| (2nf(x) \rho_{k,i}, S_{0,i}, S_{1,i}, S_{2,i}) - (\xi_k \sum_{l=1}^k E_\ell, \tilde{S}^{(m)}_{0,i}, \tilde{S}^{(m)}_{1,i}, \tilde{S}^{(m)}_{2,i})\Big\|_{TV} \,\notag\\
%&+& \|\,(\xi_k \sum_{l=1}^k E_\ell, \tilde{S}^{(m)}_{0,i},\tilde{S}^{(m)}_{1,i},\tilde{S}^{(m)}_{2,i}) - (\xi_k \sum_{l=1}^k E_\ell, \tilde{S}^{(\infty)}_{0,i},\tilde{S}^{(\infty)}_{1,i},\tilde{S}^{(\infty)}_{2,i})\,\|_{TV} \,\notag\\
%&=& \Big\| (2nf(x) \rho_{k,i}, S_{0,i}, S_{1,i}, S_{2,i}) - (\xi_k \sum_{l=1}^k E_\ell, \tilde{S}^{(m)}_{0,i}, \tilde{S}^{(m)}_{1,i}, \tilde{S}^{(m)}_{2,i})\Big\|_{TV} \,\notag\\
%&+& \|\,( \tilde{S}^{(m)}_{0,i},\tilde{S}^{(m)}_{1,i},\tilde{S}^{(m)}_{2,i}) - ( \tilde{S}^{(\infty)}_{0,i},\tilde{S}^{(\infty)}_{1,i},\tilde{S}^{(\infty)}_{2,i})\,\|_{TV} \,\notag\\
%&\stackrel{n \rightarrow \infty}{\longrightarrow}& 0 \label{eq:converge}\;,
%\end{eqnarray}
and we show that both terms converge to zero for any $m = \Theta(\log n)$.
Given that $\bh$ is continuous and bounded, this implies that
\begin{eqnarray*}
	\lim_{n\to\infty} \E[H_1|X_1 = x] &=& \E[\lim_{n\to\infty} \bh(S^{(n)})-\log f(x)|X_1 = x] \\
	&=& -\log f(x) + \E[\bh(\tS^{(\infty)})]\;,
\end{eqnarray*}
for almost every $x$, proving \eqref{eq:entropy4}.




%and $\bar{h}$ is a fixed function. Therefore, RHS is only depend on $k$. Let it be $C_{k}$, then we know that $\lim_{n \to \infty} \E[H_i | X_i = x] = - \log f(x) + C_{k}$.

The convergence of the first term follows from Lemma \ref{lem:order_stat}.
Precisely, consider the function $g_{m}: \mathbb{R}^{d \times m} \to \mathbb{R}^d \times \mathbb{R} \times \mathbb{R}^d \times \mathbb{R}^{d \times d}$ defined as:
\begin{eqnarray}
g_{m}(t_1, t_2, \dots, t_{m}) = \left(\, t_k, \sum_{j=1}^{m} \exp\{-\frac{\|t_j\|^2}{2\|t_k\|^2}\}, \sum_{j=1}^{m} \frac{t_j}{\|t_k\|} \exp\{-\frac{\|t_j\|^2}{2\|t_k\|^2}\}, \sum_{j=1}^{m} \frac{t_j t_j^T}{\|t_k\|^2} \exp\{-\frac{\|t_j\|^2}{2\|t_k\|^2}\} \,\right) \;,
\end{eqnarray}
such that $S^{(n)} = g_{m} \left(\, (c_dnf(x))^{1/d} \left(\, Z_{1,i}, Z_{2,i}, \dots, Z_{m,i} \,\right) \,\right)$
, which follows from the definition of
$S^{(n)}=((c_dnf(x))^{1/d}Z_{k,i},S_{0,i},S_{1,i},S_{2,i})$ in \eqref{eq:defS}.
Similarly,
%For $\alpha \in \{0, 1, 2\}$, define random variables
%\begin{eqnarray}
%\tilde{S}^{(m)}_{\alpha,i} = \sum_{j=1}^{m} \frac{(\xi_j\sum_{l=1}^j E_{\ell})^{\alpha}}{|\,\xi_k \sum_{l=1}^k E_\ell\,|^{\alpha}} \exp\{- \frac{(\,\sum_{l=1}^j E_{\ell}\,)^{2}}{2(\,\sum_{l=1}^k E_\ell\,)^{2}}\} \label{eq:S}\;,\\
%\tilde{T}^{(m)}_{\alpha,i} = \sum_{j=m+1}^{\infty} \frac{(\xi_j\sum_{l=1}^j E_{\ell})^{\alpha}}{|\,\xi_k \sum_{l=1}^k E_\ell\,|^{\alpha}} \exp\{- \frac{(\,\sum_{l=1}^j E_{\ell}\,)^{2}}{2(\,\sum_{l=1}^k E_\ell\,)^{2}}\} \label{eq:T}\;,
%\end{eqnarray}
%such that
 $\tS^{(m)} = g_{m} \left(\, \xi_1 E_1^{1/d}, \xi_2(E_1 + E_2)^{1/d}, \dots \xi_{m}(\sum_{\ell=1}^{m} E_\ell)^{1/d} \,\right)$.
 %$\tS^{(\infty)}\tilde{S}^{(m)}_{\alpha,i} + \tilde{T}^{(m)}_{\alpha,i} = \tilde{S}^{(\infty)}_{\alpha,i}$.
 Since $g_{m}$ is continuous, so for any set $A \in \mathbb{R}^d \times \mathbb{R} \times \mathbb{R}^d \times \mathbb{R}^{d \times d}$, there exists a set $\tA \in \mathbb{R}^{d \times m}$ such that $g_{m}(\tA) = A$. So for any $x$ such that there exists $\varepsilon > 0$ such that $f(a) > 0$, $\|\nabla f(a)\| = O(1)$ and $\|H_f(a)\| = O(1)$ for any $\|a - x\| < \varepsilon$, we have:
\begin{align}
& d_{\rm TV} ( S^{(n)},\tS^{(m)})  \,\notag\\
&= \sup_{A } %\sup_{A \in \mathbb{R}^d \times \mathbb{R} \times \mathbb{R}^d \times \mathbb{R}^{d \times d}}
\left|\, \Pr\left\{g_{m} \left(\, (c_dnf(x))^{\frac1d} Z_{1,i},  \dots, (c_dnf(x))^{\frac1d}Z_{m,i} \,\right) \in A \right\} -
	\Pr\{g_{m} (\, \xi_1 E_1^{\frac1d}, \dots \xi_{m}(\sum_{l=1}^{m} E_{\ell})^{\frac1d} \,) \in A \} \,\right| \,\notag\\
&\leq \sup_{\tA \in \mathbb{R}^{d \times m}} \left|\, \Pr\left\{\left(\, (c_dnf(x))^{1/d} Z_{1,i},  \dots, (c_dnf(x))^{1/d} Z_{m,i} \,\right) \in \tA \right\} - \Pr\{(\, \xi_1 E_1^{1/d},  \dots \xi_{m} (\sum_{\ell=1}^{m} E_\ell)^{1/d} \,) \in \tA \} \,\right| \,\notag\\
&= d_{\rm TV}\left( \left(\, (c_dnf(x))^{1/d} Z_{1,i},  \dots, (c_dnf(x))^{1/d} Z_{m,i} \,\right) \,,\, \left(\, \xi_1 E_1^{1/d}, \dots \xi_{m} (\sum_{\ell=1}^{m} E_\ell)^{1/d} \,\right)\,\right)  \,\notag\\
	&\stackrel{n \rightarrow \infty}{\longrightarrow} 0 \label{eq:converge_1}\;,
\end{align}
where the last inequality follows from Lemma \ref{lem:order_stat}. By the assumption that $f$ has open support and $\|\nabla f\|$ and $\|H_f\|$ is bounded almost everywhere, this convergence holds for almost every $x$.




For the second term in \eqref{eq:entropy3},
let $\tilde{T}^{(m)}_{\alpha} = \tS^{(\infty)}_\alpha - \tS^{(m)}_\alpha$ and
we claim that $\tilde{T}^{(m)}_{\alpha}$ converges to 0 in distribution by the following lemma.
\begin{lemma}
    \label{lem:tail}
    Assume $m \to \infty$ as $n \to \infty$ and $k\geq 3$ , %and $\tilde{T}^{(m)}_{\alpha,i}$ defined as in~\eqref{eq:T},
    then % we know that:
    \begin{eqnarray}
    \lim_{n \to \infty} \E \|\, \tilde{T}^{(m)}_{\alpha} \,\| = 0
    \end{eqnarray}
    for any $\alpha \in \{0,1,2\}$. Hence $(\tilde{T}^{(m)}_{0},\tilde{T}^{(m)}_{1},\tilde{T}^{(m)}_{2})$ converges to $(0,0,0)$ in distribution.
\end{lemma}
%Since $\tilde{S}^{(m)}_{\alpha,i} = \tilde{S}^{(\infty)}_{\alpha,i} - \tilde{T}^{(m)}_{\alpha,i}$ for any $\alpha \in \{0,1,2\}$, we know that
This implies that  $(\tilde{S}^{(m)}_{0},\tilde{S}^{(m)}_{1},\tilde{S}^{(m)}_{2})$ converges to $(\tilde{S}^{(\infty)}_{0},\tilde{S}^{(\infty)}_{1},\tilde{S}^{(\infty)}_{2})$ in distribution, i.e.,
\begin{eqnarray}
%\|\,(\tilde{S}^{(m)}_{0,i},\tilde{S}^{(m)}_{1,i},\tilde{S}^{(m)}_{2,i}) - (\tilde{S}^{(\infty)}_{0,i},\tilde{S}^{(\infty)}_{1,i},\tilde{S}^{(\infty)}_{2,i})\,\|_{TV}
d_{\rm TV}(\tS^{(m)},\tS^{(\infty)}) \stackrel{n \rightarrow \infty}{\longrightarrow} 0 \label{eq:converge_2}\;,
\end{eqnarray}







Combine~\eqref{eq:converge_1} and ~\eqref{eq:converge_2} in \eqref{eq:entropy3}, this implies the desired claim.

%Notice that $(\xi_k \sum_{l=1}^k E_\ell, \tilde{S}^{(\infty)}_{0,i}, \tilde{S}^{(\infty)}_{1,i}, \tilde{S}^{(\infty)}_{2,i})$ is a random variable depends only on $k$ (not on $n$ or underlying pdf $f(x)$). So we know that $(2nf(x) \rho_{k,i}, S_{0,i}, S_{1,i}, S_{2,i})$ converges to $(\xi_k \sum_{l=1}^k E_\ell, \tilde{S}^{(\infty)}_{0,i}, \tilde{S}^{(\infty)}_{1,i}, \tilde{S}^{(\infty)}_{2,i})$ in distribution.

We next prove the upper bound on the variance, following the technique from \cite[Section 7.3]{BD16}.
 For the usage of Efron-Stein inequality, we need a second set of i.i.d. samples $\{X'_1, X'_2, \dots, X'_n\}$. For simplicity, denote $\hH = \hH_{kLNN}^{(n)}(X)$ be the kLNN estimate base on original sample $\{X_1, \dots, X_n\}$ and $\hH^{(i)}$ be the kLNN estimate based on $\{X_1, \dots, X_{i-1}, X'_i, X_{i+1}, \dots X_n\}$. Then Efron-Stein theorem states that
\begin{eqnarray}
\Var \left[ \hH \right] \leq 2 \sum_{j=1}^n  \mathbb{E} \left[\, \left( \hH - \hH^{(j)} \right)^2 \,\right] \;.\label{eq:efron_stein}
\end{eqnarray}

Recall that
\begin{eqnarray*}
	\hH = \frac1n \sum_{i=1}^n \Big\{ \underbrace{\bh\big(\,(c_d nf(X_i))^{1/d} Z_{k,i}, S_{0,i}, S_{1,i}, S_{2,i})\,\big) - \log f(X_i)}_{\equiv H_i}  \Big\} \;,
\end{eqnarray*}
where  $\bar{h} : \mathbb{R}^d \times \mathbb{R} \times \mathbb{R}^d \times \mathbb{R}^{d \times d} \to [-10^{10}, 10^{10}]$ is defined from
\begin{align}
&h(t_1, t_2, t_3, t_4) = \nonumber\\
&\;\;d \log \|t_1\| + d \log (2 \pi) - \log c_d - \log t_2  + \frac{1}{2} \log \left(\, \det\left(\, \frac{t_4}{t_2} - \frac{t_3 t_3^T}{t^2_2}\,\right) \,\right)+ \frac{1}{2} t_3^T (t_4 - t_3 t_3^T)^{-1} t_3 \;,
\end{align}
and $\bar{h} = h$ if $|h| < 10^{10}$, $\bar{h} = 10^{10}$ if $h > 10^{10}$ and $\bar{h} = -10^{10}$ if $h < -10^{10}$. 
 Similarly, we can write $\hH^{(j)} = \frac1n \sum_{i=1}^n H_i^{(j)}$ for any $j \in \{1, \dots, n\}$. Therefore, the difference of $\hH$ and $\hH^{(j)}$ can be bounded by:
\begin{eqnarray}
 \hH - \hH^{(j)} = \frac{1}{n} \sum_{i=1}^n \left(\, H_i - H_i^{(j)} \,\right) \;.
\end{eqnarray}

Notice that $H_i$ only depends on $X_i$ and its $m$ nearest neighbors, so $H_i - H_i^{(j)} = 0$ if none of $X_j$ and $X'_j$ are in $m$ nearest neighbor of $X_i$. If we denote $Z_{i,j} = \mathbb{I} \{X_j \textrm{ is in } m \textrm{ nearest neighbor of } X_i\}$, then $H_i = H_i^{(j)}$ if $Z_{i,j}+Z_{i,j'} = 0$. According to Lemma 20.6~\cite{BD16}, since $X$ has a density, with probability one, $\sum_{i=1}^n Z_{i,j} \leq m \gamma_d$, where $\gamma_d$ is the minimal number of cones of angle $\pi/6$ that can cover $\mathbb{R}^d$, which only depends on $d$. Similarly, $\sum_{i=1}^n Z_{i,j'} \leq m \gamma_d$. If we denote $S = \{i: Z_{i,j} + Z_{i,j'} > 0\}$, the cardinality of $S$ satisfy $|S| \leq 2 m \gamma_d$. Therefore, we have $\hH - \hH^{(j)} = \frac{1}{n} \sum_{i \in S} \left(\, H_i - H_i^{(j)} \,\right)$. By Cauchy-Schwarz inequality, we have
\begin{eqnarray}
\mathbb{E} \left[\, \left( \hH - \hH^{(j)} \right)^2 \,\right] &=& \mathbb{E} \left[\, \frac{1}{n^2} \left(\, \sum_{i \in S} \left(\, H_i - H_i^{(j)} \,\right) \,\right)^2\,\right] \,\notag\\
&\leq& \mathbb{E} \left[\, \frac{|S|}{n^2} \sum_{i \in S} \left(\, H_i - H_i^{(j)} \,\right)^2\,\right] \,\notag\\
&=& \frac{|S|}{n^2} \sum_{i \in S} \mathbb{E} \left[\, \left(\, H_i - H_i^{(j)}\,\right)^2\,\right] \,\notag\\
&\leq& \frac{2|S|}{n^2} \sum_{i \in S} \left(\, \mathbb{E} \left[\, H_i^2\,\right] + \mathbb{E} \left[\, (H_i^{(j)})^2\,\right] \,\right) \;.\label{eq:h-h_j}
\end{eqnarray}

Notice that $H_i$'s and $H_i^{(j)}$'s are identically distributed, so we are left to compute $\mathbb{E} \left[\, H_1^2 \,\right]$. Conditioning on $X_1 = x$, similarly to~\eqref{eq:entropy2}, we have
\begin{eqnarray}
\E \left[\, (H_1 + \log f(x))^2 | X_1 = x\,\right] &=& \E \left[\, \bar{h}^2( (c_d nf(x))^{1/d} Z_{k,i}, S_{0,1}, S_{1,i}, S_{2,i}) \,\right] \,\notag\\
& \longrightarrow & B^{(2)}_{k,d}\;,
\end{eqnarray}
as $n \to \infty$, where $B^{(2)}_{k,d} \equiv \E\left[\, \bar{h}^2 \left(\,\xi_k \left(\, \sum_{\ell=1}^k E_\ell \,\right)^{1/d}, \tilde{S}^{(\infty)}_{0}, \tilde{S}^{(\infty)}_{1}, \tilde{S}^{(\infty)}_{2} \,\right) \,\right]$. Therefore,
\begin{eqnarray}
\E \left[\, H_1^2 | X_1 = x\,\right] &=& B^{(2)}_{k,d} - 2 \log f(x) \E \left[\, H_1 | X_1 = x\,\right] - (\log f(x))^2 \,\notag\\
&=& B^{(2)}_{k,d} - 2 \log f(x) B_{k,d} + (\log f(x))^2 \;.
\end{eqnarray}
Take expectation over $X_1$, we obtain:
\begin{eqnarray}
\E [H_1^2] &=& \E_{X_1} \left[\, \lim_{n \to \infty} \E \left[\, H_1^2 | X_1 \,\right] \,\right] = \E_{X_1} \left[\, B^{(2)}_{k,d} - 2 \log f(X_1) B_{k,d} + (\log f(X_1))^2 \,\right] \,\notag\\
&=& B^{(2)}_{k,d} + 2 H(X) B_{k,d} + \int f(x) (\log f(x))^2 dx < +\infty\;,
\end{eqnarray}
where the last inequality comes from the assumption that $\int f(x) (\log f(x))^2 dx < +\infty$. Combining with~\eqref{eq:efron_stein} and~\eqref{eq:h-h_j}, we have
\begin{eqnarray}
\Var \left[ \hH \right] \leq 2 \sum_{j=1}^n  \mathbb{E} \left[\, \left( \hH - \hH^{(j)} \right)^2 \,\right] \leq\frac{4|S|}{n} \sum_{i \in S} \left(\, \mathbb{E} \left[\, H_i^2\,\right] + \mathbb{E} \left[\, (H_i^{(j)})^2\,\right] \,\right) \leq \frac{8|S|^2 C_2}{n} \leq \frac{32m^2 \gamma_d^2 C_2}{n} \;,
\end{eqnarray}
where $C_2$ is the upper bound for $\E [H_1^2]$. Take $m = O(\log n)$ then the proof is complete.




% ------------------------------------------------------------------------------------------------------------------------------------------------

\subsection{Proof of Lemma~\ref{lem:tail}}

Firstly, since $|\xi_i| = 1$, we can upper bound the expectation of $\E \|\, \tilde{T}^{(m)}_{\alpha,i} \,\|$ by:
\begin{eqnarray}
\E \|\, \tilde{T}^{(m)}_{\alpha,i} \,\| &=& \E \, \Big\|\, \sum_{j=m+1}^{\infty} \frac{\xi_j^{(\alpha)} (\sum_{\ell=1}^j E_{\ell})^{\alpha/d}}{(\sum_{\ell=1}^k E_\ell)^{\alpha/d} } \exp\{- \frac{(\,\sum_{\ell=1}^j E_\ell\,)^{2/d}}{2(\,\sum_{\ell=1}^k E_\ell\,)^{2/d}}\} \Big\|\, \,\notag\\
&\leq& \sum_{j=m+1}^{\infty} \E \,\Big\|\, \frac{ \xi_j^{(\alpha)} (\sum_{\ell=1}^j E_{\ell})^{\alpha/d} }{(\sum_{\ell=1}^k E_\ell)^{\alpha/d} } \exp\{- \frac{(\,\sum_{\ell=1}^j E_{\ell}\,)^{2/d}}{2(\,\sum_{\ell=1}^k E_\ell\,)^{2/d}}\} \,\Big\| \,\notag\\
&=& \sum_{j=m+1}^{\infty} \E \,\Big|\, \frac{(\sum_{\ell=1}^j E_{\ell})^{\alpha/d}}{(\,\sum_{\ell=1}^k E_\ell\,)^{\alpha/d}} \exp\{- \frac{(\,\sum_{\ell=1}^j E_{\ell}\,)^{2/d}}{2(\,\sum_{\ell=1}^k E_\ell\,)^{2/d}}\} \,\Big|\;. \label{eq:eq1}
\end{eqnarray}
Notice that the expression is a function of $(\sum_{\ell=1}^j E_{\ell}/\sum_{\ell=1}^k E_{\ell})^{1/d} \equiv R_j$ for $j > m$, we will identify the distribution of $R_j$ first. For any fixed $j \geq k$, let $T_k = \sum_{\ell=1}^k E_{\ell}$ and $T_{j-k} = \sum_{\ell=k+1}^j E_{\ell}$, such that $R_j = ((T_k + T_{j-k})/T_k)^{1/d}$. Notice that $T_k$ is the summation of $k$ i.i.d. standard exponential random variables, so $T_k \sim \textit{ Erlang } (k,1)$. Similarly, $T_{j-k} \sim \textit{ Erlang }(j-k,1)$. Also $T_k$ and $T_{j-k}$ are independent. Recall that the pdf of $\textit{ Erlang }(k, \lambda)$ is given by $f_{k,\lambda}(x) = \lambda^k x^{k-1} e^{-\lambda x}/(k-1)!$ for $x \geq 0$. Therefore, the CDF of $R_j$ is given by:
\begin{eqnarray}
F_{R_j}(t) &=& \Pr \{R_j \leq t\} = \Pr\{ (\frac{T_k + T_{j-k}}{T_k})^{1/d} \leq t\} = \Pr \{\frac{T_{j-k}}{T_k} \leq t^d - 1\} \,\notag\\
&=& \int_{x \geq 0} \frac{x^{k-1} e^{-x}}{(k-1)!} \left(\, \int_{y=0}^{(t^d-1)x} \frac{y^{j-k-1}e^{-y}}{(j-k-1)!} dy \,\right) dx \,\notag\\
&=& \int_{x \geq 0} \frac{x^{k-1} e^{-x}}{(k-1)!} \left(\, 1 - \sum_{\ell=0}^{j-k-1} \frac{1}{\ell!} x^{\ell} (t^d-1)^{\ell} e^{-x(t^d-1)} \,\right) dx \,\notag\\
&=& 1 - \sum_{\ell=0}^{j-k-1} \left(\, \int_{x \geq 0} \frac{x^{k-1}e^{-x}}{(k-1)!} \frac{1}{\ell!} x^{\ell}(t^d-1)^{\ell} e^{-x(t^d-1)} dx\,\right) \,\notag\\
&=& 1 - \sum_{\ell=0}^{j-k-1} \left(\, \frac{(t^d-1)^{\ell}}{(k-1)! \ell!} \int_{x \geq 0} x^{k-1+\ell} e^{-xt^d} dx\,\right) \,\notag\\
&=& 1 - \sum_{\ell=0}^{j-k-1} \frac{(t^d-1)^{\ell}}{(k-1)! \ell!} \,(k-1+\ell)! \,t^{-d(k-1+\ell)} \,\notag\\
&=& 1- \sum_{\ell=0}^{j-k-1} {k-1+\ell \choose \ell} \, t^{-d(k-1)} (1-t^{-d})^{\ell} \;,
\end{eqnarray}
for $t \in [1,+\infty)$. Given the CDF of $R_j$, each term in~\eqref{eq:eq1} is upper bounded by:
\begin{eqnarray}
&& \E \,\Big|\, \frac{(\sum_{\ell=1}^j E_{\ell})^{\alpha/d}}{(\,\sum_{\ell=1}^k E_\ell\,)^{\alpha/d}} \exp\{- \frac{(\,\sum_{\ell=1}^j E_{\ell}\,)^{2/d}}{2(\,\sum_{\ell=1}^k E_\ell\,)^{2/d}}\} \,\Big| = \E_{R_j} \Big|\, t^{\alpha} e^{-t^2} \,\Big| \leq \E_{R_j} \left[\, t^{2} e^{-t^2} \,\right] \,\notag\\
&=& \int_{t=1}^{\infty} t^2 e^{-t^2} dF_{R_j}(t)= t^2 e^{-t^2} F_{R_j}(t) \Big|_{1}^{\infty} - \int_{t=1}^{\infty} F_{R_j}(t) d(t^2 e^{-t^2}) \,\notag\\
&=& - \int_{t=1}^{\infty} (2te^{-t^2} - 2t^3 e^{-t^2}) F_{R_j}(t) dt = \int_{t=1}^{\infty} 2t(t^2-1)e^{-t^2} F_{R_j}(t) dt \;. \label{eq:eq2}
\end{eqnarray}
Therefore, in order to establish an upper bound for~\eqref{eq:eq1}, we need an upper bound for $F_{R_j}(t)$. Here we will consider two cases depending on $t$. If $t > (j/2k)^{1/d}$, we just use the trivial upper bound $F_{R_j}(t) < 1$. If $1 \leq t \leq (j/2k)^{1/d}$, since $t^d \geq 1$, we have:
\begin{eqnarray}
F_{R_j}(t) = 1- \sum_{\ell=0}^{j-k-1} {k-1+\ell \choose \ell} \, t^{-d(k-1)} (1-t^{-d})^{\ell} \leq 1- \sum_{\ell=0}^{j-k-1} {k-1+\ell \choose \ell} \, t^{-dk} (1-t^{-d})^{\ell} \;.
\end{eqnarray}
Notice that ${k-1+\ell \choose \ell} \, t^{-dk} (1-t^{-d})^{\ell}$ is the pmf of negative binomial distribution ${\rm NB}(k, 1-t^{-d})$. Therefore, $F_{R_j}(t) \leq \Pr\{ X \geq j-k\}$, where $X \sim {\rm NB}(k, 1-t^{-d})$. The mean and variance of $X$ are given by $\E[X] = (1-t^{-d})k/(1-(1-t^{-d})) = (t^d-1)k$ and ${\rm Var}(X) = (1-t^{-d})k/(1-(1-t^{-d}))^2 = (t^{2d}-t^d)k$. Therefore, by Chebyshev inequality, the tail probability is upper bounded by:
\begin{eqnarray}
\Pr\{ X \geq j-k \} \leq \frac{{\rm Var}(X)}{(j-k-\E[X])^2} = \frac{(t^{2d}-t^d)k}{(j-k-(t^d-1)k)^2} = \frac{(t^{2d}-t^d)k}{(j-t^dk)^2} \leq 4t^{2d}k/j^2 \;,
\end{eqnarray}
here we use the fact that $t \leq (j/2k)^{1/d}$ so $j - t^dk > j/2$. Therefore, $F_{R_j}(t) \leq 4t^{2d}k/j^2$ for $t > (j/2k)^{1/d}$. Combine the two cases and plug into~\eqref{eq:eq2}, we obtain:
\begin{eqnarray}
&& \E \,\Big|\, \frac{(\sum_{\ell=1}^j E_{\ell})^{\alpha/d}}{(\,\sum_{\ell=1}^k E_\ell\,)^{\alpha/d}} \exp\{- \frac{(\,\sum_{\ell=1}^j E_{\ell}\,)^{2/d}}{2(\,\sum_{\ell=1}^k E_\ell\,)^{2/d}}\} \,\Big| = \int_{t=1}^{\infty} 2t(t^2-1)e^{-t^2} F_{R_j}(t) dt \,\notag\\
&\leq& \int_{t=1}^{(j/2k)^{1/d}} 2t(t^2-1) e^{-t^2} \frac{4t^{2d}k}{j^2} dt + \int_{(j/2k)^{1/d}}^{\infty} 2t(t^2-1) e^{-t^2} dt \,\notag\\
&\leq& \frac{8k}{j^2} \int_{t=1}^{\infty} t^{2d+3} e^{-t^2} dt + 2 \int_{(j/2k)^{1/d}}^{\infty} t^3 e^{-t^2} dt \,\notag\\
&\leq& \frac{8k C_{d}}{j^2} + 2 \left(\, -\frac{1}{2}e^{-t^2}(t^2+1) \Big|_{(j/2k)^{1/d}}^{\infty}\,\right) \,\notag\\
&=& \frac{8k C_{d}}{j^2} + e^{-(j/2k)^{2/d}} ((\frac{j}{2k})^{2/d}+1) \;,
\end{eqnarray}
where $C_d = \int_{t=1}^{\infty} t^{2d+3} e^{-t^2} dt$ is a constant only depend on $d$. Therefore, we can see that
\begin{eqnarray}
\E \,\Big|\, \frac{(\sum_{\ell=1}^j E_{\ell})^{\alpha/d}}{(\,\sum_{\ell=1}^k E_\ell\,)^{\alpha/d}} \exp\{- \frac{(\,\sum_{\ell=1}^j E_{\ell}\,)^{2/d}}{2(\,\sum_{\ell=1}^k E_\ell\,)^{2/d}}\} \,\Big| = O(1/j^2).
\end{eqnarray}
 So
\begin{eqnarray}
\E \|\, \tilde{T}^{(m)}_{\alpha,i} \,\| &\leq& \sum_{j=m+1}^{\infty} \E \,\Big|\, \frac{(\sum_{\ell=1}^j E_{\ell})^{\alpha/d}}{(\,\sum_{\ell=1}^k E_\ell\,)^{\alpha/d}} \exp\{- \frac{(\,\sum_{\ell=1}^j E_{\ell}\,)^{2/d}}{2(\,\sum_{\ell=1}^k E_\ell\,)^{2/d}}\} \,\Big| \to 0\;. \label{eq:eq1}
\end{eqnarray}
given $m \to \infty$ as $n \to \infty$.

% ------------------------------------------------------------------------------------------------------------------------------------------------------
\section{Proof of Theorem \ref{thm:unify}}
\label{sec:proof_unify}

The proposed estimator is a solution to a maximization problem $\ha = \arg\max_a \cL_{X_i}(f_{a,X_i})$.
From \cite{Loa96}  we know that the maximizer is a fixed point of a series of non-linear equations of the form
\begin{eqnarray*}
	&&\sum_{j\neq i}  \frac{(X_j-X_i)^{ \otimes \alpha }}{\rho_{k,i}^{\alpha}} K\Big( \frac{X_j-X_i}{\rho_{k,i}} \Big) \\
	&&=\;\;n \,\rho_{k,i}^d \,e^{a_0} \int  \frac{(u-X_i)^{ \otimes \alpha }}{\rho_{k,i}^{\alpha}} K\Big( \frac{u-X_i}{\rho_{k,i}} \Big)
	e^{\<u-x,a_1\> + \cdots + a_p[(u-x),\cdots,(u-x)]}   \frac{1}{\rho_{k,i}^{d}} \,du
\end{eqnarray*}
for all $\alpha\in[p]$
where the superscript $\otimes\alpha$ indicates the $\alpha$-th order tensor product.
From the proof of Theorem \ref{thm:unbiased}, specifically \eqref{eq:converge_1} and \eqref{eq:converge_2},
we know that the left-hand side converges to a value that only depends on $k,d$ and $K$.
Let's denote it by $S_\alpha(k)\in\reals^{d^\alpha}$.
We make a change of variables $\ta_0=a_0+d\log \rho_{k,i} + \log n$
and $\ta_\alpha=a_\alpha/\rho_{k,i}^\alpha$ for $\alpha\neq 0$.
Then, in the limit of growing $n$, the above equations can be rewritten as
\begin{eqnarray}
	S_\alpha(k,d,K) &=& e^{\ta_0} F_\alpha(d,K,\ta_1,\ldots,\ta_p) \;,
\end{eqnarray}
for some function $F_\alpha$. Notice that the dependence on the underlying distribution vanishes in the limit,
and the fixed point $\ta$ only depends on $k$, $p$, $d$, and $K$. The desired claim follows from the fact that
the estimate is $\lim_{n\to \infty} \hf_n(X_i)=\lim_{n\to \infty}e^{\ha_0} =  \lim_{n\to \infty}A_{k,d,p,K}/(n \rho_{k,i}^d)=
f(X_i)A_{k,d,p,K}C_d \lim_{n}1 / (C_d n \rho_{k,i}^d f(X_i)) = f(X_i)A_{k,d,p,K}C_d /\sum_{\ell=1}^k E_\ell $,  and plugging in the entropy estimator
$\hH(X) \to E_{X_i}[-\log f(X_i)]+B_{k,d,p,K} $.

In the case of the KL estimator, it happens that
$S_0=k$ and $F_0(d)=C_d$ such that $e^{\ta_0}=k/C_d$,
$e^{\ha_0} = f(X_i) k/(C_d \rho_{k,i}^d f(X_i)n)$ and $B_{k,d,p,K} = -\log k + E[\log (\sum_{\ell=1}^k E_\ell)] = -\log k + \phi(k)$.








